Agnostic Sharpness-Aware Minimization

Sharpness-aware minimization (SAM) has been instrumental in improving deep neural network training by minimizing both the training loss and the sharpness of the loss landscape, leading the model into flatter minima that are associated with better generalization properties. In another aspect, Model-Agnostic Meta-Learning (MAML) is a framework designed to improve the adaptability of models. MAML optimizes a set of meta-models that are specifically tailored for quick adaptation to multiple tasks with minimal fine-tuning steps and can generalize well with limited data. In this work, we explore the connection between SAM and MAML in enhancing model generalization. We introduce Agnostic-SAM, a novel approach that combines the principles of both SAM and MAML. Agnostic-SAM adapts the core idea of SAM by optimizing the model toward wider local minima using training data, while concurrently maintaining low loss values on validation data. By doing so, it seeks flatter minima that are not only robust to small perturbations but also less vulnerable to data distributional shift problems. Our experimental results demonstrate that Agnostic-SAM significantly improves generalization over baselines across a range of datasets and under challenging conditions such as noisy labels or data limitation.

==> rebuttal/review__4HkJ_score4.tex <==
\subsection{Summary}
The paper proposes Agnostic Sharpness-aware minimization (SAM), an approach combining the principle of SAM and Model-agnostic Meta Learning (MAML). This approach essentially optimizes a model towards wider minima using training data while maintaining a low loss on validation data. The authors claim that this makes the model less vulnerable to distribution shift. Experiments demonstrate that Agnostic SAM outperforms SGD and SAM on small image classification datasets.


\subsection{Strengths}
The approach is sound, theoretically grounded and quite novel.
The presentation is clear, however there are a few issues remain.

\subsection{Weaknesses}

\begin{itemize}
    \item Agnostic SAM requires longer training time than SAM, although it seems to produce better results.
\item Agnostic SAM requires more hyperparameters to tune, such as $\rho_1$, $\rho_2$, $|B^t|$ and $|B^v|$
\item The experiments lack comparisons to other variants of SAM such as ASAM.
\item No experiments on larger datasets, such as ImageNet.
\item There are many typos in the papers, the most serious one is the wrong caption in Table 5.
\item Small numbers to select for tuning SAM hyperparams. The authors need to do a more thorough jobs on hyperparameter tuning for the baselines.

\item The caption of Table 3 does not mention which metric is used in the table.
No experiment demonstrating that Agnostic SAM improves model robustness to distribution shift, despite the claim made in the abstract.
\end{itemize}

\subsection{Questions}
\begin{itemize}
    \item Theorem 2 states that Agnostic SAM makes the gradient on  $|B_v|$ more aligned with that of $|B^t|$. Could you show that this actually happen in the experiments?
    \item Could you provide comparisons to another variants of SAM such as ASAM?
    \item Can you confirm that Agnostic SAM also benefits from m-sharpness like SAM?
\end{itemize}





==> rebuttal/reviewer_MM77_score4.tex <==
\subsection{Summary}
This paper solve Model-Agnostic Machine Learning with bi-level optimization. The method is utilizing sharpness aware minimization in the outer optimization for the generalization performance.


\subsection{Strengths}

The primary results seems to work.
Good theoretical validation.

\subsection{Weaknesses}
\begin{itemize}
    \item Empirical gain on cifar-10 datasets (table) is marginal.
    \item Lack of qualitative analysis on the better generalization quality. You can do case study for correct prediction.
    \item Too expensive training costs in table 6.
    \item All the experiments are conducted on small scale. I think cifar is too small, so scalability can not be guaranteed. Adding imagenet experiments.
    \item The paper treat limited scope.
\end{itemize}

\subsection{Questions}


==> rebuttal/reviewer__HVHP_score5.tex <==
\subsection{Summary}
The paper investigates the synergy between Sharpness-aware Minimization (SAM) and Model-Agnostic Meta-Learning (MAML) to enhance the generalization of deep learning models. SAM, which promotes flatter minima for better generalization by minimizing the sharpness of the loss landscape along with the training loss, and MAML, which focuses on optimizing models for quick adaptability across multiple tasks with minimal tuning, are integrated in a novel approach called Agnostic-SAM. This new method adjusts the core concept of SAM to not only aim for wider local minima during training but also to ensure lower loss on validation data, targeting robustness against perturbations and resilience to shifts in data distribution. Experimental results show that Agnostic-SAM outperforms standard baselines, particularly under conditions such as noisy labels and limited data, thereby significantly boosting model generalization across various datasets.

\subsection{Strengths}
\begin{itemize}
    \item The idea is clear and straightforward, and the authors provide solid theoretical and empirical support to verify its effectiveness.
    \item Sharpness-Aware Minimization and Model-Agnostic Meta-Learning are two significant topics within the machine learning community. By connecting them, the authors offer new and intriguing insights that could benefit the field.
\end{itemize}

\subsection{Weaknesses}
\begin{itemize}
    \item In the empirical studies, the authors focus primarily on comparing Agnostic-SAM with SGD and SAM. To enhance the persuasiveness of their results, the inclusion of additional baselines would be beneficial.
    \item The authors claim to have attached the source code, but I am unable to locate it.
    \item In the current machine learning community, CIFAR is considered less challenging and attractive. The paper's focus on CIFAR for empirical studies may limit its relevance to real-world applications.

\end{itemize}

\subsection{Questions}
For Theorem 1, I am curious whether the new upper bound is tighter than the corresponding one in SAM, or if it is merely a general version applicable to various loss functions.



==> rebuttal/reviewer__v6KD_score4.tex <==
\subsection{Summary}
The authors proposed a novel Sharpness-aware minimization approach, called Agnostic SAM, that incorporate the principals from MAML into SAM to improve the model generalization.


\subsection{Strengths}
Agnostic SAM not only seeks flatter minima but is less vulnerable to data distribution shift problems.

\subsection{Weaknesses}
The main weakness of the current paper is its weak experimental section. Paper is ignoring newer baselines and important datasets and is based on the flatness assumption for generalization that is argued by many papers to be a weak hypothesis. Methods like [1, 2, 3, 4] show that the sharpness metric induced by SAM does not necessarily correlate with generalization in modern deep learning architectures.

[1] Andriushchenko, M., Croce, F., Mu ̈ller, M., Hein, M., and Flammarion, N. A modern look at the relationship between sharpness and generalization. arXiv preprint arXiv:2302.07011, 2023b.

[2] Kaur, S., Cohen, J., and Lipton, Z. C. On the maximum hessian eigenvalue and generalization. In Proceedings on, pp. 51–65. PMLR, 2023.

[3] Mueller, M., Vlaar, T., Rolnick, D., and Hein, M. Normalization layers are all that sharpness-aware minimization needs. arXiv preprint arXiv:2306.04226, 2023.

[4] Baek, C., Kolter, J. Z., and Raghunathan, A. Why is SAM robust to label noise? In The Twelfth International Conference on Learning Representations, 2024.

Regarding the baselines the authors only compare Agnostic SAM with SAM. Nevertheless, newer, and stronger baselines like GSAM [5], ASAM [cited by authors but not compared] and more recently OBF [6] should also be benchmarked since they are the current state-of-the-art.
[5] Zhuang, J., Gong, B., Yuan, L., Cui, Y., Adam, H., Dvornek, N., Tatikonda, S., Duncan, J., and Liu, T. Surrogate gap minimization improves sharpness-aware training. arXiv preprint arXiv:2203.08065, 2022.

[6] Vani, A; Tung, F; Oliveira G; Sharifi H. ”Forget Sharpness: Perturbed Forgetting of Model Biases Within SAM Dynamics”, International Conference on Machine Learning (ICML) 2024.

Another point to improve is the datasets used, none of the used datasets are large scale. I strongly suggest the authors to benchmark with at least a couple large scale datasets. Options are ImageNet-V1 [7] for training and ImageNet-Real [8] and ImageNet-V2 [9] for testing, ImageNet-R [10] for out-of-distribution robustness benchmark and ImageNet-Sketch [11].
[7] Deng, J., Dong, W., Socher, R., Li, L.-J., Li, K., and Fei-Fei, L. ImageNet: A large-scale hierarchical image database. In 2009 IEEE conference on computer vision and pattern recognition, pp. 248–255. IEEE, 2009

[8] Beyer, L., He ́naff, O. J., Kolesnikov, A., Zhai, X., and Oord, A. v. d. Are we done with imagenet? arXiv preprint arXiv:2006.07159, 2020.

[9] Recht, B., Roelofs, R., Schmidt, L., and Shankar, V. Do imagenet classifiers generalize to imagenet? In Interna- tional conference on machine learning, pp. 5389–5400. PMLR, 2019.

[10] Hendrycks, D., Basart, S., Mu, N., Kadavath, S., Wang, F., Dorundo, E., Desai, R., Zhu, T., Parajuli, S., Guo, M., et al. The many faces of robustness: A critical analysis of out-of-distribution generalization. In Proceedings of the IEEE/CVF International Conference on Computer Vision, pp. 8340–8349, 2021.

[11] Wang, H., Ge, S., Lipton, Z., and Xing, E. P. Learning robust global representations by penalizing local predictive power. In Advances in Neural Information Processing Systems, pp. 10506–10518, 2019.

\subsection{Questions}
As referred on the weakness section I revision on related works, benchmarks and datasets will be needed to bring the paper to a stronger state.


==> rebuttal/reviewer_o2hn_score3.tex <==
\subsection{Summary}
The authors present a variant of SAM based on MAML. The authors propose modifying the SAM perturbation step to include an additional term that ensures that loss on a validation set remains low. The authors motivate their algorithm with a PAC-Bayes bound. They provide experimental validation of their algorithm.

\subsection{Strengths}
The paper observes an interesting connection between SAM and MAML, and presents a theoretically motivated algorithm. Further, the authors present empirical evidence that their algorithm can improve performance in multiple settings.

\subsection{Weaknesses}
One major weakness of this paper is its lack of clarity \& rigor for the theoretical claims.
\begin{itemize}
    \item Theorem 1 is not formally stated; the authors do not explain the assumptions of the theorem (neither in the main paper nor the appendix).
    \item Important notation is not defined: the definition of (e.g., Eq. 1) is not provided. Further, the is also not properly defined (line 107). This makes understanding the precise statement of the rest of the claims difficult.
    \item The proofs of the theorems are unclear. As one example, it's unclear how the bound on line 435 was derived. More generally, much of the paper would benefit from careful explanation of the relevant terms. Also, be sure to carefully check the paper for typos. The main weakness of the empirical claims are that in most cases, the and batch size parameters are not tuned. Both parameters have a substantial impact on the performance of SAM (see e.g., Figure 1 of [1]). The authors should tune the baselines over both parameters for all experiments to properly demonstrate that their algorithm outperforms those baselines.
\end{itemize}
[1] Andriushchenko, Maksym, and Nicolas Flammarion. "Towards understanding sharpness-aware minimization." International Conference on Machine Learning. PMLR, 2022.

==> section/ablation_study_old.tex <==
\section{Ablation Study}

\subsection{Experiments on various setting of AgnosticSAM}

\textbf{Split training and validation set.}
Theoretically, the training and validation sets are independent and identically distributed samples from the data distribution. However, due to the limited number of available samples, splitting the original training set into two non-overlapping subsets for training $S^t$ and validation $S^v$ notably reduces the number of training samples. This reduction can make it challenging to train a deep neural network, particularly on small-size datasets like FGVC-Aircraft, and Flower102. To mitigate this, in practice, we randomly sample a mini-batch $B \sim S$ and then divide it into $B^t$ and $B^v$ with a ratio $|B^t| = r|B|$ and $|B^v| = (1-r)|B|$ in each iteration. As a result, the validation samples in $B^v$ may have been training samples in a previous iteration and the model is updated using the full training set. This approach significantly enhances the performance of Agnostic-SAM. Throughout all experiments, we use a fixed value of $r=0.7$ and use the same hyperparameters as mentioned in Section \ref{subsec:from_scratch}.

However, if we strictly follow the theoretical framework, where we split the original training set $S$ into two fixed training sets $S^t$ and validation set $S^v$ with $|S^t| = r|S|$ and $|S^v| = (1-r)|S|$, the algorithm still outperforms the baselines, even with considerably fewer training data. To demonstrate this, we conduct experiments under two settings: Agnostic-SAM (Non-overlap), which split $S=S^t \cup S^v$, and proposed Agnostic-SAM, which split $B=B^t \cup B^v$. Both settings use the same split ratio $r=0.7$.

In Figure \ref{fig:non-overlap-split}, we present a comparative analysis of SAM and the two variants of Agnostic-SAM on CIFAR-100 (on the left) and FGVC-Aircraft (on the right). Agnostic-SAM shows notable improvement over its Non-overlap version, especially on the small-size FGVC-Aircraft dataset. However, even the Non-overlap version of Agnostic-SAM consistently outperforms SAM in most experiments.

\begin{figure}[h!]

     \centering
     \begin{subfigure}
         \centering
         \includegraphics[width=0.49\textwidth]{figures/Cifar100_NonOverlapSv.png}
         % \caption{SWA and F-S}
         % \label{fig:y equals x}
     \end{subfigure}
     % \hfill
     \begin{subfigure}
         \centering
         \includegraphics[width=0.49\textwidth]{figures/Aircraft_Nonoverlap.png}
         % \caption{$y=3\sin x$}
         % \label{fig:three sin x}
     \end{subfigure}
     % \hfill
     \centering
     
    \caption{Comparision of setting Agnostic-SAM (Non-overlap), proposed Agnostic-SAM, and the baseline SAM on CIFAR-100 (on the left) and FGVC-Aircraft (on the right)}
     \label{fig:non-overlap-split}
     
\end{figure}



\begin{table}[h]
\centering
\caption{Experiments of AgnosticSAM and its simple version on CIFAR dataset.}

\label{tab:simpler-agnostic}
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{llccc}
% \midrule
Dataset                   & Method                       & WideResnet28x10 & Pyramid101 & Densenet121 \\ \midrule \midrule

% CIFAR-10  & SGD                         & 96.50 $\pm$ 0.100           & 96.00 $\pm$  0.100      & -    \\
\textbf{CIFAR-10}  &  SAM                         & 96.72 $\pm$ 0.007           & 96.20 $\pm$  0.134      & 91.16  $\pm$  0.240     \\
                          % & \multicolumn{1}{l}{OT-MDR}& 96.97 $\pm$ 0.009           & \textbf{96.61  $\pm$ 0.063}      & \textbf{91.44  $\pm$ 0.113}      \\
                          &  \multicolumn{1}{l}{Agnostic-SAM (Simpler) } &  96.93  $\pm$ 0.021  &  96.26  $\pm$ 0.101 & \textbf{91.46  $\pm$ 0.154}  \\ 
                          &  \multicolumn{1}{l}{Agnostic-SAM}  &  \textbf{97.17 $\pm$ 0.014}  &  \textbf{96.30 $\pm$ 0.070}  & 91.17 $\pm$ 0.148   \\ \midrule
% CIFAR-100 & SGD                         & 81.20 $\pm$  0.200           & 80.30 $\pm$  0.300     & -      \\ 
\textbf{CIFAR-100}  & SAM                         & 82.69 $\pm$  0.035           & 81.26 $\pm$  0.636      & 68.09 $\pm$  0.403       \\ 
                          % & \multicolumn{1}{l}{OT-MDR} &\textbf{ 84.14  $\pm$ 0.172}           & 82.28  $\pm$ 0.183      & \textbf{69.84  $\pm$ 0.176}       \\ 
                          &  \multicolumn{1}{l}{Agnostic-SAM (Simpler) }  &  83.36 $\pm$  0.065  &  82.27 $\pm$  0.311 &  68.97 $\pm$  0.212 \\
                          &  \multicolumn{1}{l}{Agnostic-SAM}  &  \textbf{83.86 $\pm$ 0.077}  &  \textbf{82.93 $\pm$ 0.247} &  \textbf{69.65 $\pm$ 0.226} \\ \bottomrule
\end{tabular}
}
\end{table}

\textbf{Effectiveness of sharpness on validation set.}
As presented in Section \ref{subsec:solution}, we first find the perturbed model $\tilde{\theta}_{l}^{v}$ by maximizing the loss on validation samples $B^v$, formula (\ref{eq:perturbBv}), then inject the gradient $\nabla_{\theta}\mathcal{L}_{B^{v}}\left(\tilde{\theta}_{l}^{v}\right)$ when find the actual perturbed model $\tilde{\theta}_{l}^{t}$, formula (\ref{eq:perturb_BtBv}). In this way, the actual perturbed model $\tilde{\theta}_{l}^{t}$ maximizes the loss on training samples $B^t$ and minimizes the sharpness on $B^v$ at the same time. While the proposed method is very effective in enhancing the robustness and generalization error by minimizing sharpness on both training and validation samples, it takes extra training time per epoch.

In this section, we provide a simpler version, in which, the injected gradient when finding the actual perturbed model $\tilde{\theta}_{l}^{t}$ is $\nabla_{\theta}\mathcal{L}_{B^{v}}\left(\theta_{l}\right)$. So that, the simpler version does not require extra steps to perturb the model on validation samples $B^v$ and the formula (\ref{eq:perturb_BtBv}) becomes: 

\[
\tilde{\theta}_{l}^{t} & =\theta_{l}+\eta_{1}\nabla_{\theta}\mathcal{L}_{B^{t}}\left(\theta_{l}\right)-\eta_{2}\nabla_{\theta}\mathcal{L}_{B^{v}}\left(\theta_{l}\right)
\]

In Table \ref{tab:simpler-agnostic}, we present experiments with a simpler version of Agnostic-SAM on the CIFAR dataset using various architectures. Impressively, this version consistently outperforms the baseline SAM across all settings by significant margins and achieves results comparable to those of the proposed Agnostic-SAM approach. This demonstrates the effectiveness of our method, which uses the gradient of validation samples as a guide to identify a perturbed model.

\subsection{Computation complexity}

The training times for SAM and Agnostic-SAM are presented in Table \ref{tab:training-time}. All variations of Agnostic-SAM approach require additional computational steps to calculate the gradients on the validation set in each iteration, compared to SAM. However, in the Non-overlap version, we divide the original training set $S$ into a training set $S^t$ and a validation set  $S^v$ with ratio $|S^t|=0.7|S|$ and $|S^v|=0.3|S|$, the number of training samples for this version is significantly fewer than the other methods. As a result, the training time per epoch for SAM is slightly longer than for Agnostic-SAM (Non-overlap), but considerably shorter than the other variations of Agnostic-SAM. For different versions of Agnostic-SAM, as the number of gradient steps per epoch increases, both the training time and performance tend to rise accordingly. Considering this is a trade-off for computational complexity and performance in our method.

\begin{table}[]
\centering
\caption{Compare training time (in minutes) per epoch between SAM and Agnostic-SAM on CIFAR-100 and FGVC Aircraft dataset.}

\label{tab:training-time}
\begin{tabular}{lccc}
Method                             & \textbf{WideResnet28x10} & \textbf{Pyramid101} & \textbf{Densenet121} \\ \midrule \midrule
SAM                                & 2.90 $\pm$ 0.01           & 1.75 $\pm$ 0.00      & 1.40 $\pm$ 0.04       \\
Agnostic-SAM (Non-overlap) & 2.86 $\pm$ 0.00  &   1.72  $\pm$ 0.01     & 1.25 $\pm$ 0.02    \\
Agnostic-SAM (Simpler)     & 3.56   $\pm$ 0.04          & 	2.05 $\pm$ 0.01  &	1.90 $\pm$ 0.01        \\
Agnostic-SAM                       & 4.78  $\pm$ 0.02          & 2.86  $\pm$ 0.00     & 2.25 $\pm$ 0.02      \\ \midrule
                            & \textbf{EfficientNet-B4} & \textbf{EfficientNet-B3} & \textbf{ResNet18} \\ \midrule \midrule
SAM                                &      1.41 $\pm$ 0.02     &  1.18 $\pm$ 0.01     &    0.72 $\pm$ 0.03  \\
Agnostic-SAM (Non-overlap)      & 1.42  $\pm$ 0.03    &  1.15 $\pm$ 0.00     &    0.72 $\pm$ 0.01   \\
Agnostic-SAM (Simpler)     & 1.75 $\pm$ 0.01      &	1.38 $\pm$ 0.00    &	0.96  $\pm$ 0.01      \\
Agnostic-SAM                       &     2.36  $\pm$ 0.02       &  1.71 $\pm$ 0.01      &  1.13 $\pm$ 0.00  \\ \bottomrule
\end{tabular}
\end{table}


==> section/framework_old.tex <==
\section{Proposed Framework}
\subsection{Notions}
We start with introducing the notions used throughout our paper. We denote $\mathcal{D}$ as the data/label distribution to generate pairs of data/label $(x,y)$. Given a model with the model parameter $\theta$, we denote the per sample loss induced by $(x,y)$ as $\ell(x,y;\theta)$. Let $S$ be the training set drawn from the distribution $\mathcal{D}$. We denote the empirical and general losses as $\mathcal{L}_{S}\left(\theta\right)=\mathbb{E}_{S}\left[\ell\left(x,y;\theta\right)\right]$ and $\mathcal{L}_{\mathcal{D}}\left(\theta\right)=\mathbb{E}_{\mathcal{D}}\left[\ell\left(x,y;\theta\right)\right]$ respectively. Moreover, we define $\mathcal{L}_{\mathcal{D}}\left(\theta\mid S\right)$ as an \textit{upper bound defined over $S$} of the general loss $\mathcal{L}_{\mathcal{D}}\left(\theta\right)$. Note that inspired by SAM~\citep{foret2021sharpnessaware}, we use the sharpness over $S$ to define $\mathcal{L}_{\mathcal{D}}\left(\theta\mid S\right)$. Finally, we use $|A|$ to denote the cardinality of a set $A$.

\subsection{Problem Formulation}
Given a training set $S^t$ whose examples are sampled from $\mathcal{D}$ (i.e., $S^t \sim \mathcal{D}^{N_t}$ with $N_t = |S^t|$), we use $\mathcal{L}_{\mathcal{D}}\left(\theta\mid S^{t}\right)$ to train models and among the models that minimize this loss, we select the one that minimize the general loss as follows:
\begin{equation}
\min_{\theta^{*}}\mathcal{L}_{\mathcal{D}}\left(\theta^{*}\right)\text{ s.t. }\theta^{*}\in\mathcal{A}_{\mathcal{D}}\left(S^t\right)=\text{argmin}_{\theta}\mathcal{L}_{\mathcal{D}}\left(\theta\mid S^{t}\right).\label{eq:formulation}
\end{equation}

The reason for the formulation in (\ref{eq:formulation}) is that although $\mathcal{L}_{\mathcal{D}}\left(\theta\mid S^{t}\right)$ is an upper bound of the general loss $\mathcal{L}_{\mathcal{D}}\left(\theta\right)$, there always exists a gap between them. Therefore, the additional outer minimization helps to refine the solutions. We now denote $S^v$ (i.e., $S^v \sim \mathcal{D}^{N_v}$ with $N_v = |S^v|$) as a valid set sampled from $\mathcal{D}$. With respect to this valid set, we have the following theorem.

\begin{theorem} \label{theo:1}
Denote $\mathcal{L}_{\mathcal{D}}\left(\theta\mid S\right):=\max_{\theta':\Vert\theta'-\theta\Vert_{2}\leq\rho}\mathcal{L}_{S}\left(\theta'\right)$. Under some mild condition similar to SAM \citep{foret2021sharpnessaware}, with a probability greater than $1 - \delta$ (i.e., $\delta \in [0,1]$) over the choice of $S^v \sim \mathcal{D}^{N_v}$, we then have for any optimal models $\theta^* \in \mathcal{A}_{\mathcal{D}}(S^t)$:
\begin{equation}
\mathcal{L}_{\mathcal{D}}\left(\theta^{*}\right)\leq\mathcal{L}_{\mathcal{D}}\left(\theta^{*}\mid S^{v}\right)+\frac{4L}{\sqrt{N_{v}}}\left[k\log\left(1+\frac{\Vert\theta^*\Vert^{2}}{\rho}\left(1+\sqrt{\log N_{v}/k}\right)\right)+2\sqrt{\log\frac{N_{v}+k}{\delta}}+O(1)\right]\label{eq:PAC_bound},
\end{equation}
where $L$ is the upper-bound of the loss function (i.e., $\ell\left(x,y;\theta\right)\leq L,\forall x,y,\theta$), $k$ is the model size, and $\rho>0$ is the perturbation radius.
\end{theorem}

Our theorem \ref{theo:1} (proof can be found in Appendix \ref{sec:proofs}) can be viewed as an extension of Theorem 1 in \cite{foret2021sharpnessaware}, where we apply the Bayes-PAC theorem from \cite{PAC_Bayes} to prove an upper bound for the general loss of any bounded loss, instead of the 0-1 loss in \cite{foret2021sharpnessaware}. Moreover, we can generalize this proof for $S^t$ to explain why using $\mathcal{L}_{\mathcal{D}}\left(\theta\mid S^{t}\right):=\max_{\theta':\Vert\theta'-\theta\Vert_2\leq \rho}\mathcal{L}_{S^{t}}\left(\theta'\right)$ as an objective to minimize, as in (\ref{eq:formulation}). Thanks to Theorem \ref{theo:1}, we can rewrite the objectives in (\ref{eq:formulation}) as: 
\begin{equation}
\min_{\theta^{*}}\mathcal{L}_{\mathcal{D}}\left(\theta^{*}\mid S^{v}\right)\text{ s.t. \ensuremath{\theta^{*}}\ensuremath{\in\mathcal{A}_{\mathcal{D}}\left(S^{t}\right)=\text{argmin}_{\theta}\,\mathcal{L}_{\mathcal{D}}}\ensuremath{\left(\theta\mid S^{t}\right)}},\label{eq:reformulation}
\end{equation}
where $\mathcal{L}_{\mathcal{D}}\left(\theta\mid S\right):=\max_{\theta':\Vert\theta'-\theta\Vert_{2}\leq\rho}\mathcal{L}_{S}\left(\theta'\right)$. 
\subsection{Our Solution}
\label{subsec:solution}
Our agnostic formulation has the same form as MAML~\citep{pmlr-v70-finn17a}, developed for meta-learning. Inspired by MAML, a naive approach is to consider $\theta^* = \theta^*(\theta)$ and then minimize $\mathcal{L}_{\mathcal{D}}\left({\theta}^*\left(\theta\right)\mid S^{v}\right)$ with respect to $\theta$. However, this mainly optimizes the loss $\mathcal{L}_{\mathcal{D}}\left(\theta^{*}\left(\theta\right)\mid S^{v}\right)$ over the validation set $S^v$, which is not appropriate for our motivation, where we aim to primarily optimize the loss over the training set $S^t$, while using $S^v$ to further enhance the generalization ability.  

We interpret the bi-level optimization problem in (\ref{eq:reformulation}) as follows: at each iteration, our primary objective is to optimize $\mathcal{L}_{\mathcal{D}}\left(\theta\mid S^{t}\right)$, primarily based on its gradients, in such a way that future models are able to implicitly perform well on $S^v$. To achieve this, similar to SAM \citep{foret2021sharpnessaware}, we approximate $\mathcal{L}_{\mathcal{D}}\left(\theta\mid S^{t}\right)=\max_{\Vert\theta'-\theta\Vert\leq\rho}\mathcal{L}_{S^{t}}\left(\theta'\right)\approx\mathcal{L}_{S^{t}}\left(\theta+\eta_{1}\nabla\mathcal{L}_{S^{t}}\left(\theta\right)\right)$ for a sufficient small learning rate $\eta_1>0$ (i.e., $\eta_{1}\Vert\nabla\mathcal{L}_{S^{t}}\left(\theta\right)\Vert\leq\rho$) and $\mathcal{L}_{\mathcal{D}}\left(\theta\mid S^{v}\right)=\max_{\Vert\theta'-\theta\Vert\leq\rho}\mathcal{L}_{S^{v}}\left(\theta'\right)\approx\mathcal{L}_{S^{v}}\left(\theta+\eta_{2}\nabla\mathcal{L}_{S^{v}}\left(\theta\right)\right)$ for a sufficient small learning rate $\eta_2>0$ (i.e., $\eta_{2}\Vert\nabla\mathcal{L}_{S^{v}}\left(\theta\right)\Vert\leq\rho$). 

Moreover, at each iteration, while primarily using the gradients of $\mathcal{L}_{\mathcal{D}}\left(\theta\mid S^{t}\right)$ for optimization, we also utilize the gradient of $\mathcal{L}_{\mathcal{D}}\left(\theta\mid S^{v}\right)$ in an auxiliary manner to ensure congruent behavior between these two gradients. Specifically, at the $l$-th iteration, we update as follows:
\begin{align}\tilde{\theta}_{l}^{v} & =\theta_{l}+\eta_{2}\nabla_{\theta}\mathcal{L}_{B^{v}}\left(\theta_{l}\right), \label{eq:perturbBv} \\
\tilde{\theta}_{l}^{t} & =\theta_{l}+\eta_{1}\nabla_{\theta}\mathcal{L}_{B^{t}}\left(\theta_{l}\right)-\eta_{2}\nabla_{\theta}\mathcal{L}_{B^{v}}\left(\tilde{\theta}_{l}^{v}\right), \label{eq:perturb_BtBv} \\
\theta_{l+1} & =\theta_{l}-\eta\nabla_{\theta}\mathcal{L}_{B^{t}}\left(\tilde{\theta}_{l}^{t}\right), \label{eq:update_new}
\end{align}
where $\eta_1>0,\eta_2>0$, and $\eta>0$ are the learning rates, while $\mathcal{L}_{B^{t}}\left(\theta_{l} \right)$ and $\mathcal{L}_{B^{v}}\left(\theta_{l}\right)$ represent the empirical losses over the mini-batches $B^t \sim S^t$ and $B^v \sim S^v$ respectively. 

According to the update in (\ref{eq:update_new}) (i.e., $\theta_{l+1}=\theta_{l}-\eta\nabla_{\theta}\mathcal{L}_{B^{t}}\left(\tilde{\theta}_{l}^{t}\right)$), $\theta_{l+1}$ is updated to minimize $\mathcal{L}_{B^{t}}\left(\tilde{\theta}_{l}^{t}\right)$. We now do first-order Taylor expansion for $\mathcal{L}_{B^{t}}\left(\tilde{\theta}_{l}^{t}\right)$ as 
\begin{equation}
\mathcal{L}_{B^{t}}\left(\tilde{\theta}_{l}^{t}\right)=\mathcal{\mathcal{L}}_{B_{t}}\left(\theta_{l}\right)+\eta_{1}\Vert\nabla_{\theta}\mathcal{L}_{B^{t}}\left(\theta_{l}\right)\Vert_{2}^{2}-\eta_{2}\nabla_{\theta}\mathcal{L}_{B^{t}}\left(\theta_{l}\right)\cdot\nabla_{\theta}\mathcal{L}_{B^{v}}\left(\tilde{\theta}_{l}^{v}\right),\label{eq:taylor}
\end{equation}
where $\cdot$ specifies the dot product.

From (\ref{eq:taylor}), we reach the conclusion that the update in (\ref{eq:update_new}) (i.e., $\theta_{l+1}=\theta_{l}-\eta\nabla_{\theta}\mathcal{L}_{B^{t}}\left(\tilde{\theta}_{l}^{t}\right)$) aims to \textit{minimize} simultaneously (i) $\mathcal{\mathcal{L}}_{B_{t}}\left(\theta_{l}\right)$, (ii) $\Vert\nabla_{\theta}\mathcal{L}_{B^{t}}\left(\theta_{l}\right)\Vert_{2}^{2}$, and \textit{maximize} (iii) $\nabla_{\theta}\mathcal{L}_{B^{t}}\left(\theta_{l}\right)\cdot\nabla_{\theta}\mathcal{L}_{B^{v}}\left(\tilde{\theta}_{l}^{v}\right)$. While the effects in (i) and (ii) are similar to SAM \citep{foret2021sharpnessaware}, maximizing $\nabla_{\theta}\mathcal{L}_{B^{t}}\left(\theta_{l}\right)\cdot\nabla_{\theta}\mathcal{L}_{B^{v}}\left(\tilde{\theta}_{l}^{v}\right))$ encourages two gradients of the losses over $B^t$ and $B^v$ to become more congruent. 
\begin{theorem}
    \label{theo:congruent}
    For sufficiently small learning rates $\eta_{1}\leq\frac{\left|\nabla_{\theta}\mathcal{\mathcal{L}}_{B_{t}}\left(\theta_{l}\right)\cdot\nabla_{\theta}\mathcal{L}_{B^{v}}\left(\tilde{\theta}_{l}^{v}\right)\right|}{12\left|\nabla_{\theta}\mathcal{L}_{B^{v}}\left(\tilde{\theta}_{l}^{v}\right)^{T}H_{B^{t}}\left(\theta_{l}\right)\nabla_{\theta}\mathcal{L}_{B^{t}}\left(\theta_{l}\right)\right|}$ and $\eta_{2}\leq\min\left\{ \frac{\left|\nabla_{\theta}\mathcal{\mathcal{L}}_{B_{t}}\left(\theta_{l}\right)\cdot\nabla_{\theta}\mathcal{L}_{B^{v}}\left(\tilde{\theta}_{l}^{v}\right)\right|}{6\left|\nabla_{\theta}\mathcal{L}_{B^{v}}\left(\tilde{\theta}_{l}^{v}\right)^{T}H_{B^{t}}\left(\theta_{l}\right)\nabla_{\theta}\mathcal{L}_{B^{v}}\left(\tilde{\theta}_{l}^{v}\right)\right|},\frac{\left|\nabla_{\theta}\mathcal{\mathcal{L}}_{B_{t}}\left(\theta_{l}\right)\cdot\nabla_{\theta}\mathcal{L}_{B^{v}}\left(\tilde{\theta}_{l}^{v}\right)\right|}{6\left|\nabla_{\theta}\mathcal{L}_{B^{v}}\left(\tilde{\theta}_{l}^{v}\right)^{T}H_{B^{v}}\left(\tilde{\theta}_{l}^{v}\right)\nabla_{\theta}\mathcal{L}_{B^{t}}\left(\theta_{l}\right)\right|}\right\} $, we have
    \begin{equation}
\nabla_{\theta}\mathcal{L}_{B^{t}}\left(\tilde{\theta}_{l}^{t}\right)\cdot\nabla_{\theta}\mathcal{L}_{B^{v}}\left(\tilde{\theta}_{l}^{v}\right)\geq\begin{cases}
\frac{1}{2}\nabla_{\theta}\mathcal{L}_{B^{t}}\left(\theta_{l}\right)\cdot\nabla_{\theta}\mathcal{L}_{B^{v}}\left(\tilde{\theta}_{l}^{v}\right) & \text{if}\,\nabla_{\theta}\mathcal{L}_{B^{t}}\left(\theta_{l}\right)\cdot\nabla_{\theta}\mathcal{L}_{B^{v}}\left(\tilde{\theta}_{l}^{v}\right)\geq0\\
\frac{3}{2}\nabla_{\theta}\mathcal{L}_{B^{t}}\left(\theta_{l}\right)\cdot\nabla_{\theta}\mathcal{L}_{B^{v}}\left(\tilde{\theta}_{l}^{v}\right) & \text{otherwise}
\end{cases}\label{eq:inequality}
\end{equation}
\end{theorem}

Theorem \ref{theo:congruent} (proof can be found in Appendix \ref{sec:proofs}) indicates that two gradients $\nabla_{\theta}\mathcal{L}_{B^{t}}\left(\tilde{\theta}_{l}^{t}\right)$ and $\nabla_{\theta}\mathcal{L}_{B^{v}}\left(\tilde{\theta}_{l}^{v}\right)$ are encouraged to be more congruent since our update aims to maximize its lower bound $c\times\nabla_{\theta}\mathcal{L}_{B^{t}}\left(\theta_{l}\right)\cdot\nabla_{\theta}\mathcal{L}_{B^{v}}\left(\tilde{\theta}_{l}^{v}\right)$ (i.e., $c=0.5$ or $c=1.5$). Notice that the negative gradient $-\eta\nabla_{\theta}\mathcal{L}_{B^{t}}\left(\tilde{\theta}_{l}^{t}\right)$ is used to update $\theta_l$ to $\theta_{l+1}$, hence this update can have implicit impact on minimizing $\mathcal{L}_{\mathcal{D}}\left(\theta\mid S^{v}\right)$ since the negative gradient $-\nabla_{\theta}\mathcal{L}_{B^{v}}\left(\tilde{\theta}_{l}^{v}\right)$ targets to minimize $\mathcal{L}_{\mathcal{D}}\left(\theta\mid S^{v}\right)=\max_{\Vert\theta'-\theta\Vert\leq\rho}\mathcal{L}_{S^{v}}\left(\theta'\right)\approx\mathcal{L}_{S^{v}}\left(\theta+\eta_{2}\nabla\mathcal{L}_{S^{v}}\left(\theta\right)\right)$. 

\paragraph{Practical Algorithm.} For the practical Agnostic-SAM algorithm, inspired by SAM \citep{foret2021sharpnessaware}, we replace $\eta_{1}=\rho_{1}\frac{\nabla_{\theta}\mathcal{L}_{B^{t}}\left(\theta_{l}\right)}{\Vert\nabla_{\theta}\mathcal{L}_{B^{t}}\left(\theta_{l}\right)\Vert_{2}}$ and $\eta_{2}=\rho_{2}\frac{\nabla_{\theta}\mathcal{L}_{B^{v}}\left(\tilde{\theta}_{l}^{v}\right)}{\Vert\nabla_{\theta}\mathcal{L}_{B^{v}}\left(\tilde{\theta}_{l}^{v}\right)\Vert_{2}}$, where $\rho_1>0$ and $\rho_2>0$ are perturbation radii. Furthermore, instead of using two fixed sets $S^t$ and $S^v$, and then sampling mini-batches $B^t \sim S^t$ and $B^v \sim S^v$, we employ an on-the-fly strategy. Specifically, let $S$ be the entire training set (e.g., $S=S^{t}\cup S^{v}$), we sample a mini-batch $B \sim S$ and then split it into $B^t$ and $B^v$ (e.g., $|B^t| = 0.7|B|$ and $|B^v| = 0.3|B|$). The pseudo-code of Agnostic-SAM is summarized in Algorithm \ref{alg:agnosticSAM}. 


\begin{algorithm}
    \caption{Pseudo-code of Agnostic-SAM}\label{alg:agnosticSAM}
    \begin{algorithmic}
    \State \textbf{Input:} $\rho_1, \rho_2, \eta$, the number of iterations $L_{\text{iter}}$, and the training set $S$.
    \State \textbf{Output:} the optimal model $\theta_L$.
    \For{$l=1$ to $L_{\text{iter}}$}
        \State Sample mini-batch $B \sim S$.
        \State Randomly split $B$ to $B^t$ and $B^v$.
        \State Compute $\tilde{\theta}_{l}^{v}=\theta_{l}+\rho_{2}\frac{\nabla_{\theta}\mathcal{L}_{B^{v}}\left(\theta_{l}\right)}{\Vert\nabla_{\theta}\mathcal{L}_{B^{v}}\left(\theta_{l}\right)\Vert_{2}}$.
        \State Compute $\tilde{\theta}_{l}^{t}=\theta_{l}+\rho_{1}\frac{\nabla_{\theta}\mathcal{L}_{B^{t}}\left(\theta_{l}\right)}{\Vert\nabla_{\theta}\mathcal{L}_{B^{t}}\left(\theta_{l}\right)\Vert_{2}}-\rho_{2}\frac{\nabla_{\theta}\mathcal{L}_{B^{v}}\left(\tilde{\theta}_{l}^{v}\right)}{\Vert\nabla_{\theta}\mathcal{L}_{B^{v}}\left(\tilde{\theta}_{l}^{v}\right)\Vert_{2}}$.
        \State Compute $\theta_{l+1}=\theta_{l}-\eta\nabla_{\theta}\mathcal{L}_{B^{t}}\left(\tilde{\theta}_{l}^{t}\right)$.
    \EndFor
    \end{algorithmic}
\end{algorithm}



 





